Rotation-Adaptive Point Cloud Domain Generalization via Intricate Orientation Learning

The vulnerability of 3D point cloud analysis to unpredictable rotations poses an open yet challenging problem: orientation-aware 3D domain generalization. Cross-domain robustness and adaptability of 3D representations are crucial but not easily achieved through rotation augmentation. Motivated by the inherent advantages of intricate orientations in enhancing generalizability, we propose an innovative rotation-adaptive domain generalization framework for 3D point cloud analysis. Our approach aims to alleviate orientational shifts by leveraging intricate samples in an iterative learning process. Specifically, we identify the most challenging rotation for each point cloud and construct an intricate orientation set by optimizing intricate orientations. Subsequently, we employ an orientation-aware contrastive learning framework that incorporates an orientation consistency loss and a margin separation loss, enabling effective learning of categorically discriminative and generalizable features with rotation consistency. Extensive experiments and ablations conducted on 3D cross-domain benchmarks firmly establish the state-of-the-art performance of our proposed approach in the context of orientation-aware 3D domain generalization.

==> figure_tsne.tex <==
\begin{figure*}[t]
    % \flushleft
    \centering
    \subfloat[Baseline]{%[b]{0.45\textwidth}
        \label{fig:tsne_randrot}
        % \centering
        \includegraphics[width=0.24\textwidth]{./resources/visualization/randrot.pdf}
        % \vspace{10mm}
    }
    \subfloat[Ours]{%[b]{0.45\textwidth}
        \label{fig:tsne_ours}
        % \centering
        \includegraphics[width=0.24\textwidth]{./resources/visualization/ours.pdf}
        % \vspace{10mm}
    }
    \subfloat[Ablation of $\lambda_{oc}$]{%[b]{0.45\textwidth}
        \label{fig:plot_lambda_oc}
        % \centering
        \includegraphics[width=0.24\textwidth]{./resources/visualization/ablation_cons_weights.pdf}
        % \vspace{10mm}
    }
    \subfloat[Ablation of $\lambda_{ms}$]{%[b]{0.45\textwidth}
        \label{fig:plot_lambda_ms}
        % \centering
        \includegraphics[width=0.24\textwidth]{./resources/visualization/ablation_reg_weights.pdf}
        % \vspace{10mm}
    }
    \vspace{-1mm}
    \caption{T-SNE visualizations of the features for class \textcolor[RGB]{0,47,167}{"plant"}, \textcolor[RGB]{153,102,204}{"sofa"} and \textcolor[RGB]{240,0,86}{"chair"} on $M\to S$ are presented in (a) and (b), where the $\cdot$ and $\times$ denote source domain and target domain, respectively. The curves of performance under varying $\lambda_{oc}$ and $\lambda_{ms}$ are post in (c) and (d).}
    \label{fig:visualization}
    \vspace{-6mm}
\end{figure*} 

==> table_complexity.tex <==

\begin{table}[h]
    \caption{Time statistics (ms) of training/testing on one batch of data.}
    \label{tab:complexity}
    \vspace{-3ex}
    \small
    \begin{center}
    \setlength{\tabcolsep}{0.4cm}{
    \resizebox{0.4\textwidth}{!}{
      \begin{tabular}{c|c|c|c|c} 
        \hline 
        Methods & Type & Avg. & $T_{train}$& $T_{test}$ \\
        \hline
        VN~\cite{Deng_2021_ICCV} & RE & 41.3 & 808 & 27.9 \\
        SPRIN~\cite{you2021prin} & RI & 43.9 & 1551 & 370.2 \\
        RIPCA~\cite{li2021closer} & RI & 46.6 & 717 & 23.3 \\
        MLSP~\cite{liang2022point} & DA & 43.2 & 825 & 36.5 \\
        SDDA~\cite{cardace2023self} & DA & 43.1 & \bf{567} & \bf{12.0} \\
        \hline
        Ours & DG & \bf{49.6} & 2114 & 14.5 \\
        \hline
        \end{tabular}
    }
    }
    \end{center}
  \end{table}
  
